Tricking Retrievers with Influential Tokens: An Efficient Black-Box Corpus Poisoning Attack

Retrieval-augmented generation (RAG) systems enhance large language models by incorporating external knowledge, addressing issues like outdated internal knowledge and hallucination. However, their reliance on external knowledge bases makes them vulnerable to corpus poisoning attacks, where adversarial passages can be injected to manipulate retrieval results. Existing methods for crafting such passages, such as random token replacement or training inversion models, are often slow and computationally expensive, requiring either access to retriever's gradients or large computational resources. To address these limitations, we propose Dynamic Importance-Guided Genetic Algorithm (DIGA), an efficient black-box method that leverages two key properties of retrievers: insensitivity to token order and bias towards influential tokens. By focusing on these characteristics, DIGA dynamically adjusts its genetic operations to generate effective adversarial passages with significantly reduced time and memory usage. Our experimental evaluation shows that DIGA achieves superior efficiency and scalability compared to existing methods, while maintaining comparable or better attack success rates across multiple datasets.

==> latex/tables/results2.tex <==
\begin{table*}[htbp]
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{c>{\centering\arraybackslash}p{2.3cm}*{6}{c}}
\toprule
\multirow{3}{*}[-3pt]{\textbf{Dataset}} & \multirow{3}{*}[-3pt]{\textbf{Method}} & \multicolumn{6}{c}{\textbf{Number of Adversarial Passages}} \\
\cmidrule(lr){3-8}
& & \multicolumn{2}{c}{\textbf{1}} & \multicolumn{2}{c}{\textbf{10}} & \multicolumn{2}{c}{\textbf{50}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
& & \textbf{ASR@5} & \textbf{ASR@20} & \textbf{ASR@5} & \textbf{ASR@20} & \textbf{ASR@5} & \textbf{ASR@20} \\
\midrule
\multirow{6}{*}[-3pt]{NQ} 
& \multicolumn{7}{c}{\textit{White-box Methods}} \\
\cmidrule(lr){2-8}
& HotFlip   & 0.1 & 1.3 & 0.4 & 3.2 & 2.0 & 9.6 \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\textit{Black-box Methods}} \\
\cmidrule(lr){2-8}
& Vec2Text  & 0.0 & 0.0 & 0.7 & 2.4 & 2.8 & 8.1 \\
& \textbf{DISA (ours)} & 0.0 & 0.0 & 0.2 & 1.9 & 1.4 & 5.3 \\
\midrule
\multirow{6}{*}[-3pt]{NFCorpus}
& \multicolumn{7}{c}{\textit{White-box Methods}} \\
\cmidrule(lr){2-8}
& HotFlip  & 37.2 & 58.8 & 44.6 & 68.1 & 47.7 & 71.2 \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\textit{Black-box Methods}} \\
\cmidrule(lr){2-8}
& Vec2Text  & 0.6 & 2.5 & 8.1 & 14.2 & 23.0 & 38.7 \\
& \textbf{DISA (ours)}    & 5.7 & 10.8 & 11.2 & 18.2 & 26.1 & 44.3 \\
\midrule
\multirow{6}{*}[-3pt]{FIQA}
& \multicolumn{7}{c}{\textit{White-box Methods}} \\
\cmidrule(lr){2-8}
& HotFlip   & 0.5 & 1.9 & 2.5 & 7.4 & 8.5 & 25.2 \\
\cmidrule(lr){2-8}
& \multicolumn{7}{c}{\textit{Black-box Methods}} \\
\cmidrule(lr){2-8}
& Vec2Text  & 0.0 & 0.0 & 0.9 & 1.2 & 3.9 & 11.9 \\
& \textbf{DISA (ours)} & 0.0 & 0.0 & 1.3 & 1.7 & 4.4 & 14.3 \\
\bottomrule
\end{tabular}
}

\begin{tabular}{ccc}
\toprule
\textbf{Method} & \textbf{Avg. Time} & \textbf{Avg. GPU Usage} \\
\midrule
HotFlip & 1.0x & -- \\
Vec2Text & -- & -- \\
\textbf{DISA (ours)} & -- & -- \\
\bottomrule
\end{tabular}

\caption{\textbf{Attack Success Rate evaluation results, with average Time and GPU usage across all datasets}}
\label{tab:comprehensive-experiment-results}
\end{table*}

==> latex/tables/sparse.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Dense Retriever}} & \multicolumn{3}{c}{\textbf{Sparse Retriever}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
\textbf{Method} & ASR@5 & ASR@20 & ASR@50 & ASR@5 & ASR@20 & ASR@50 \\
\midrule
HotFlip & 0.4 & 3.2 & 10.4 & 0.0 & 0.0 & 0.0 \\
Vec2Text & 0.7 & 2.4 & 4.2 & N/A & N/A & N/A \\
\textbf{DIGA (ours)} & & & & & & \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of Attack Success Rate (ASR) for Dense and Sparse Retrievers.} Results are shown for the Natural Questions dataset with 10 adversarial passages injected. The dense retriever and sparse retriever are GTR and BM25 respectively. N/A indicates that the method is not applicable to sparse retrievers.}
\label{tab:dense-sparse-comparison}
\end{table*}

==> latex/tables/transferability.tex <==
\begin{table*}[htbp]
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{>{\centering\arraybackslash}p{1.3cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{1.6cm}*{3}{>{\centering\arraybackslash}p{1.5cm}}>{\centering\arraybackslash}p{1.9cm}}
\toprule
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{Method}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Attack}\\\textbf{Retriever}\end{tabular}} & \multicolumn{3}{c}{\textbf{RAG Retriever}} & \multirow{3}{*}{\textbf{Transferability}} \\
\cmidrule(lr){4-6}
& & & GTR-base & ANCE & DPR-NQ & \\
\midrule
\multirow{7}{*}{NQ} & \multirow{3}{*}{HotFlip} & GTR-base &  9.6 \cellcolor{lightgray!25} & 0.0 & 0.0 & \textcolor{red}{0.0} \\
& & ANCE & 0.0 & 28.4\cellcolor{lightgray!25} & 0.0 & \textcolor{red}{0.0} \\
& & DPR-NQ & 0.0 & 0.0 & 1.7\cellcolor{lightgray!25} & \textcolor{red}{0.0} \\
\cmidrule(lr){2-7}
& Vec2Text & GTR-base & \cellcolor{lightgray!25} 8.1 & 0.0 & 0.0 & \textcolor{red}{0.0} \\
\cmidrule(lr){2-7}
& \multirow{3}{*}{\textbf{DISA (ours)}} & GTR-base & \cellcolor{lightgray!25} & & &  \\
& & ANCE & & \cellcolor{lightgray!25} & &  \\
& & DPR-NQ & & & \cellcolor{lightgray!25} &  \\
\midrule
\multirow{7}{*}{FiQA} & \multirow{3}{*}{HotFlip} & GTR-base & 25.2\cellcolor{lightgray!25} & 0.0 & 0.0 & \textcolor{red}{0.0} \\
& & ANCE & 0.0 & 81.5\cellcolor{lightgray!25} & 0.0 & \textcolor{red}{0.0} \\
& & DPR-NQ & 0.0 & 0.0 & 92.1\cellcolor{lightgray!25} & \textcolor{red}{0.0} \\
\cmidrule(lr){2-7}
& Vec2Text & GTR-base & \cellcolor{lightgray!25} 11.9 & 0.0 & 0.0 & \textcolor{red}{0.0} \\
\cmidrule(lr){2-7}
& \multirow{3}{*}{\textbf{DISA (ours)}} & GTR-base & \cellcolor{lightgray!25} & & &  \\
& & ANCE & & \cellcolor{lightgray!25} & &  \\
& & DPR-NQ & & & \cellcolor{lightgray!25} &  \\
\midrule
\multirow{7}{*}{NFCorpus} & \multirow{3}{*}{HotFlip} & GTR-base & 71.2\cellcolor{lightgray!25} & 0.0 & 0.0 & \textcolor{red}{0.0} \\
& & ANCE & 0.0 & 96.9\cellcolor{lightgray!25} & 0.0 & \textcolor{red}{0.0} \\
& & DPR-NQ & 0.0 & 0.0 & 92.9 \cellcolor{lightgray!25} & \textcolor{red}{0.0} \\
\cmidrule(lr){2-7}
& Vec2Text & GTR-base & \cellcolor{lightgray!25} 38.7 & 9.3 \textsuperscript{\color{red}$\downarrow$76.0\%} & 0.6 \textsuperscript{\color{red}$\downarrow$98.4\%} & \textcolor{green!40!black}{12.9} \\
\cmidrule(lr){2-7}
& \multirow{3}{*}{\textbf{DISA (ours)}} & GTR-base & \cellcolor{lightgray!25} & & &  \\
& & ANCE & & \cellcolor{lightgray!25} & &  \\
& & DPR-NQ & & & \cellcolor{lightgray!25} &  \\
\bottomrule
\end{tabular}
\caption{\textbf{Transferability Analysis.} The results represent the adversarial success rate (ASR@20) after injecting 50 adversarial passages. Cells with gray background denote in-domain attacks, where the same retriever used to generate adversarial passages is applied in the RAG system. For the Vec2Text model, we only include the scenario where the attack retriever is GTR-base, as the inversion model is trained on GTR embeddings. Consequently, embeddings from ANCE or DPR-NQ cannot be inverted back to text.}

\label{tab:multi_dataset_transferability}
\end{table*}

==> latex/tables/transferability_retrievers.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{lccc}
\toprule
& \multicolumn{3}{c}{\textbf{Retriever}} \\
\cmidrule(lr){2-4}
\multirow{1}{*}{\textbf{Method}} & GTR-base & ANCE & DPR-NQ \\
\midrule
HotFlip & 7.4 & 3.2 & 10.4 \\
Vec2Text & 1.2 & 2.4$^{\dagger}$ & N/A$^{\dagger}$ \\
\textbf{DIGA (ours)} & & & \\
\bottomrule
\end{tabular}
\caption{\textbf{Comparison of Attack Success Rate (ASR) for Different Retrievers. FIQA dataset} Inject 10 and evaluate ASR@20. $^{\dagger}$ marks the case where we have an incompatibility between the retriever and inversion model.}
\label{tab:retriever}
\end{table}
